Self-Supervised Beat Tracking in Musical Signals with Polyphonic Contrastive Learning

Annotating musical beats is a very long and tedious process. In order to combat this problem, we present a new self-supervised learning pretext task for beat tracking and downbeat estimation. This task makes use of Spleeter, an audio source separation model, to separate a song's drums from the rest of its signal. The first set of signals are used as positives, and by extension negatives, for contrastive learning pre-training. The drum-less signals, on the other hand, are used as anchors. When pre-training a fully-convolutional and recurrent model using this pretext task, an onset function is learned. In some cases, this function is found to be mapped to periodic elements in a song. We find that pre-trained models outperform randomly initialized models when a beat tracking training set is extremely small (less than 10 examples). When this is not the case, pre-training leads to a learning speed-up that causes the model to overfit to the training set. More generally, this work defines new perspectives in the realm of musical self-supervised learning. It is notably one of the first works to use audio source separation as a fundamental component of self-supervision.

==> CHANGES <==
Changes in version 4.2 (September 2015)
o Fixed issue between titlesec and tocloft regarding
  part numbering in the ToC (classicthesis.sty). 
	Thanks to Enrico Gregorio and Henri Menke.
o Fixed bug with colored lines and graffiti 
  (classicthesis.sty). Thanks to Enrico Gregorio and
  Stefano Bragaglia for the fix! (Also switched
  graffiti from \slshape to \itshape.)
o Changed \vspace*{8ex} to \vspace{8ex} (Contents.tex)	
o Moved \cleardoublepage from end of Contents.tex 
  to appropriate position in ClassicThesis.tex
o \bflabel of acronym package removed, as it was 
  removed from acronym package and caused errors.
  Now set \aclabelfont to \acsfont for consistency.
o Converted major files to UTF-8 (thanks to Jörn Hees)
  (Bibliography.bib excluded for now as BibTeX cannot
  handle UTF-8)
o Added support for BibLaTeX in 
  classicthesis-config.tex and Bibliography.tex
	(thanks to Jörn Hees).
	For LyX we will have a work-around for testing.
o Added an example for one's own publication list
  (via BibLaTeX) in Publications.tex (renamed from 
	Publication.tex)
o Replaced/updated scrpage2 with scrlayer-scrpage 
  in classicthesis.sty (thanks to Ivo Pletìkosić).
X Worked on Appendix case with floatperchapter 
  (works for captions but not for references so far)
	Thanks to Claus Lahiri and Clemens Niederberger 
	for their help on this.
	[REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]	
X Removed fixltx2e from classicthesis-config.tex and
  have classicthesis.sty use or emulate the latest 
	LaTeX kernel via latexrelease (option: latest)
  (thanks to Jörn Hees).
	[REMOVED AS IT IS NOT AVAILABLE IN MANY 
	DISTRIBUTIONS, SEE ISSUE #107]
	
Changes in version 4.1 (August 2012)
o Working towards XeLaTeX support:
	- "ifxetex" package for checking whether
	  XeTeX is in use (classicthesis.sty)
	- Adjusted part, chapter, and tocEntry 
	- Thanks to Joerg Weber for his ideas and code
	- Option "pdfspacing" does not work for XeTeX
	  and is disabled when XeTeX is running
	  (maybe implement spacing with fontspec later)
o Load additional packages in order to 
  reduce warnings (classicthesis-config.tex)
	- "textcomp" to fix warnings with missing font 
	  shapes
	- "scrhack" to fix warnings when using KOMA 
	  with listings package  
o Replaced \mathrm-command with \textrm-command
  (Chapter03.tex)

Changes in version 4.0 (December 2011)
o Due to lots of issues and complaints, 
  classicthesis-preamble.sty is replaced by 
  classicthesis-config.tex (which is cleaner,
  nicer, better, etc. than before!)
o No per-chapter-numbering also for equations 
  (classicthesis.sty and Chapter03.tex)
o classicthesis.sty now also works without the 
  KOMA-classes (scrbook, scrartcl, etc.):
	- This affects the text body shape, where the
	  package "typearea" is always loaded in order 
	  to use \areaset
	- And affects the layout of footnotes where the 
	  package "footmisc" is loaded otherwise
	  (not 100\% identical look-and-feel but OK)
o Help for using spanish babel with classicthesis 
  (classicthesis-config.tex)
o Note about pdfsync issues with graffiti 
  (Chapter01.tex)
o Minor clean-up of comments and duplicate lines 
  (classicthesis.sty)
o Adjusted the colophon text (Colophon.tex)
o Increased space for labels in the LoF, LoT, LoL
o Included version information on the title page and
  in the drafting and final version information 
  (classicthesis.sty and Titlepage.tex)

Changes in version 3.0 (June 2011)
o There have been some major changes in order to port 
  classicthesis to LyX easily. See below for details.
  Special thanks go to Ivo Pletikosi\'c for all his 
  hard work he put into this project!
o Changes in ClassicThesis.tex:
	- Redundant fleqn removed from documentclass options 
	 (will be set by amsmath package in preamble)
	- KOMA adjustments for documentclass: 
	  fontsize=11pt,paper=14
	- Moved language options into documentclass due to LyX
	  issues with babel
o Changes in classicthesis.sty:
	- Removed bcor from \areaset command so that it can
	  be set via \documentclass option (BCOR=)
	- New \ctparttext command for putting preamble text
	  after part titles (see ClassicThesis.tex for examples)
	- \graffito command now also available as original
	  \marginpar (backward compatibility is enabled)
	- Chapter number in margin done with \oldmarginpar
o Changes to classicthesis-preamble.sty:
  - Fixed autoref for subfigures (see Chapter 2 for example)
  - Fixed issues with redefining autoref strings (for
      different languages)
	- Now contains all configuration information, such as
	  the title, your name etc.
	- This package now also loads classicthesis.sty, change
	  the options classicthesis to be loaded with here  
	- Package inputenc now loaded with latin9 option 
	- Package listings now also loaded here
	- Now safer package loading regarding options by
	  using \PassOptionsToPackage command extensively
	- Inserted new string for \mySubtitle
o Changes in Titlepage.tex and Titleback.tex because of new 
  string \mySubtitle
o Changed a lot of the documentation, e.g., in Chapter01.tex

Changes in version 2.9 (January 2011)
o Fixed onlytext euler font for MinionPro font (in 
  classicthesis.sty)
o Option "listsseparated" deprecated, because it led to some
  strange side-effects (in classicthesis.sty)
o Changed default font size to 11pt (in ClassicThesis.tex) and
  adjusted text block size accordingly (in classicthesis.sty)
o Fixed bug with backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o New option "floatperchapter" for classicthesis.sty, removed 
  all code for that from classicthesis-ldpkg.sty
o Removed "nochapters" option from classicthesis-ldpkg.sty
o Removed redundant loading of listings package (in
  classicthesis-ldpkg.sty)
o Fixed some headline bug in example classicthesis-book.tex
o Fixed a bug when using parts with plain latex as in example
  classicthesis-book.tex (in classicthesis.sty)

Changes in version 2.8 (March/May 2010)
o Fixed serious \graffito bug in classicthesis.sty
  (thanks to Lorenzo Pantieri and Enrico Gregorio)
o Included backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o Fixed drafting issues (draft information not shown at all)
  caused by wrong code for listings and listsseparated options
  in classicthesis.sty 

Changes in version 2.7 (February 2010, cumulative release)
o Removed option for classicthesis-ldpkg.sty: nobackref 
  Introduced instead option "backref" for consistency
  which works the other way (no backrefs by default)
  
Changes in version 2.6.2 (January 2010, released as beta)
o New option for classicthesis-ldpkg.sty: nobackref 
  (removes links to cited page in bibliography)
o Fixed some spacing issues for LoF, LoT, LoL with option
  "listsseparated" (in classicthesis.sty)

Changes in version 2.6.1 (October 2009, released as beta)
o Removed \myChapter and \myPart, you can now use the regular
  \chapter and \part commands (in classicthesis.sty)
  (thanks to Hinrich Harms for this)
o Fixed used KOMA-options: numbers=noenddot, cleardoublepage=empty
  (in ClassicThesis.tex)
o Included hack to use citations in float environments, will 
  be fixed with caption package version 3.2 (in classicthesis.sty)
o Included some font and text area fine-tuning code 
  (in ClassicThesis.tex)
o Some testing with Libertine font (classicthesis-book.tex)
o Fixed numbering of listings used in different chapters
  (in ClassicThesis.tex, classicthesis.sty, classicthesis-ldpkg.sty)
o Spacing between listings in different chapters and after List 
  of Listings header fixed (in classicthesis.sty)
o Increased \newnumberwidth to sizeof(999) which is better for 
  documents with more than 99 pages (in classicthesis.sty)
o New option for classicthesis.sty: manychapters
    
Changes in version 2.6 (August 2009)
o Centered the title page with the addmargin environment
  (thanks to Nicolas Repp for the hint)
o Fixed header for page two of Table of Contents (with 3 
  or more pages) (in Contents.tex)
o Added numbering of \subsubsection (in Contents.tex)
o Added correct Table of Contents entries for \subsubsection
  (in classicthesis.sty)
o Added printonlyused option to loading acronym package
  (in classicthesis-ldpkg.sty)
o Some code for "clean" hyperlinks (w/o color and w/o boxes)
o Minor fix for \graffito (in classicthesis.sty)

Changes in version 2.5.1 (May 2009, released as beta)
o New option for classicthesis.sty: dottedtoc
  (Refer to the manual for more information.)
o New option for classicthesis.sty: listings
  (Refer to the manual for more information.)
  (Credit + thanks to Prof. Enrico Gregorio)
o Minor clean-up and bug-fixing

Changes in version 2.5 (October 2008, cumulative release)
o Increased text-width for better page layout (experimental)
o Cumulative release, some minor clean-up and bug-fixing

Changes in version 2.4.{1--3} (February and April 2008,
released as betas)
o Switched back to "obsolete" KOMA options due to 
  compatibility issues on some installations
o Increased robustness of \cauthor command in 
  classicthesis-ldpk.sty
o Spacing fix for \sectionmark (in classicthesis.sty) 
o Made Booleans private (in classicthesis.sty)
o Acronyms header for long acronym lists (in Contents.tex)
o Moved "amsmath" package from classicthesis.sty to
  ClassicThesis.tex
o "MinionPro" package now loaded with "mathlf" option
  instead of "osf" option (in classicthesis.sty)
o Fixed issue with contents headings (in classicthesis.sty
  and in Contents.tex)
o Thanks to Lorenzo

Changes in version 2.3 (November 2007)
o Fixed serious bug with \myChapter command (using plain 
  LaTeX)
o Removed hypcap package from classicthesis-ldpkg.sty and
  placeins package from classicthesis.sty. Put both into
  ClassicThesis.tex for finer end-user control
o Removed obsolete KOMA options from ClassicThesis.tex
o Option "subfigure" deprecated, replaced by "subfig" (in 
  classicthesis.sty)
o Inserted some mechanisms to detect whether subfig(ure) 
  package was loaded or not (in classicthesis.sty)
o Inserted some mechanism to detect whether classicthesis
  packackage was loaded or not (in classicthesis-ldpkg.sty)
o Moved "headlines" code block a bit up in 
  classicthesis.sty (seemed to cause problems with new
  KOMA-Script classes)
o Removed accidental "natbib" from classicthesis-ldpkg.sty  
o Some fine-tuning in (Dirty)Titlepage.tex
o Thanks to Lorenzo and Denis! :-)

Changes in version 2.2 (October 2007)
o \myChapter and \myPart now take an optional argument
  just as the regular \part and \chapter commands
o Did some minor changes to classicthesis-book.tex
  so it's a better example
o Inserted some \cleardoublepage before \myPart 
  occurences to avoid pdfbookmark problems
o Introduced some general typographic fine-tuning
  (linespread, penalties, etc.)
o Did some fine-tuning of the \graffito command

Changes in version 2.1 (July 2007)
o Removed duplicate xcolor package call from 
  classicthesis-ldpkg.sty and shifed some color
  definitions around
o Removed re-definition of \ttdefault

Changes in version 2.0 (June 2007, cumulative release)
o Better setup of the list of acronyms 
  (in classicthesis-ldpkg.sty)
o Using KOMA option footinclude in ClassicThesis.tex
  (text block sizes are adjusted to this)
o New option for classicthesis.sty: minionpro
o New option for classicthesis.sty: minionprospacing
o New option for classicthesis.sty: pdfspacing
  (Refer to the manual for more information.)

Changes in version 1.7 (May 2007, not released separately)
o Removed \graphicspath from ClassicThesis.tex
o Use the nag package to ensure "compliance"
o Switched from ccaption to caption in classicthesis-ldpkg.sty
  (setup via \captionsetup in ClassicThesis.tex)
o Switched from subfigure to subfig in classicthesis-ldpkg.sty
o Removed obsolete "usenames" option from loading xcolor package
o Noticed problem with \thelstlisting on some installations
  (commented out in classicthesis-ldpkg.sty)
o Noticed problem with some hyperlinks on some installations
  (could not determine cause)

Changes in version 1.6 (April 2007, not released separately)
o Included greetings to Lorenzo Pantieri for many very useful
  suggestions
o Introduced new commands in classicthesis-ldpkg.sty to make
  adaptation of backrefs to different languages easier
   - \backrefnotcitedstring (ref is not cited)
   - \backrefcitedsinglestring (ref is cited on one page)
   - \backrefcitedmultistring (ref is cited on multiple pages)
o Removed ellipsis package from classicthesis-ldpkg.sty due to 
  some undesired results for some users
o Removed the following packages from classicthesis-ldpkg.sty as 
  these seem to require changes to their options from most users:
  inputenc, babel, natbib (now in ClassicThesis.tex)
o New option for classicthesis-ldpkg.sty: nochapters
  Use the package with classes that do not have chapter divisions 

Changes in version 1.5 (April 2007, not released separately)
o Fixed some bugs to use classicthesis.sty for article layout
o Inserted some info/warnings when using nochapter/parts
o Extended the manual: examples for using classicthesis.sty for
  other projects than a thesis (source available in folder
  "Examples")
o Some minor adjustments in classicthesis-ldpkg.sty
o Fixed some spelling mistakes

Changes in version 1.4.2 (March 2007)
o Renamed loadpackages.sty to classicthesis-ldpkg.sty due to
  TeX Live package tree issues

Changes in version 1.4.1 (March 2007)
o Fixed some wording concerning the license :-o
o Added fixltx2e and ellipsis packages to to loadpackages.sty to correct
  some minor glitches
o Fixed and changed some things about ToC entries of parts
o Some minor bug fixes

Changes in version 1.4 (January 2007)
o Replaced \lineheight with \baselineskip in classicthesis.sty
o Removed obsolete "usenames" option from xcolor package (classicthesis.sty)
o Now classicthesis.sty processes the global a5paper option and adjusts 
  the layout accordingly (experimental!)

Changes in version 1.3.1 (August 2006)
o Urgent bug concerning ToC spacing etc. fixed

Changes in version 1.3 (August 2006) 
o New option for classicthesis.sty: parts
  Turn this on if you use Part divisions. It fine-tunes the ToC and
  adds support for Part division via \myPart{} (cf. \myChapter{})
  (The style of this feature is preliminary, any suggestions?!)
o New option for classicthesis.sty: eulermath
  Uses the awesome Euler fonts for math (Palatino fonts are default).
o Added mparhack package to loadpackages.sty to get the graffiti right
o Added a hint to loadpackages.sty on how to typeset the List of 
  Listings consistently with classicthesis
o Some minor fine-tuning of typographic details
o Collaboration with babel package improved (now easier to use
  with other languages than English)
o Added appropriate textwidth values for 11pt Palatino and Minion
  (See comments near \areaset in classicthesis.sty)
o Note: There is a problem with the case of math text in part-, 
  chapter-, and section titles and I have no clue how to fix this 
  (either the case or the spacing breaks). So far, I chose the case. :-(

Changes in version 1.2 (June 2006)
o Setup a little postcard collection: http://postcards.miede.de
o Changed stupid spelling mistake: "A Homage" => "An Homage" D'oh!
o New option for classicthesis.sty: nochapters
  Allows to use the look-and-feel with classes that do not use chapters.
o New option for classicthesis.sty: beramono
  Loads Bera Mono as typewriter font. (Default = no typewriter font.)
o Included list of files, see LISTOFFILES.  

Changes in version 1.1 (May 2006)
o classicthesis.sty now stand-alone and usable w/o whole bundle!
o classicthesis.sty compatible with both LaTeX and PDFLaTeX
  Note: this is only true for classicthesis.sty, not the whole bundle.
o New option for classicthesis.sty: subfigure
  Tells the style to add the respective option when loading tocloft.
o Now loading microtype package w/o options (classicthesis.sty)
o Fixed overfull hbox warnings for ToC entries (classicthesis.sty)
o No longer depending on a particular caption package (classicthesis.sty)
o Layout for subsubsections provided (classicthesis.sty)
o PDF opens on title page (ClassicThesis.[tex|pdf])
o Files are a bit more "ASCII-friendly" (all)
o Note: Thanks to all the folks who already sent me a postcard! :-)

Version 1.0 (March 2006)
o First public release

==> FrontBackmatter/Colophon.tex <==
\pagestyle{empty}

\hfill

\vfill


\pdfbookmark[0]{Colophon}{colophon}
\section*{Colophon}
This document was typeset using the typographical look-and-feel \texttt{classicthesis} developed by Andr\'e Miede. 
The style was inspired by Robert Bringhurst's seminal book on typography ``\emph{The Elements of Typographic Style}''. 
\texttt{classicthesis} is available for both \LaTeX\ and \mLyX: 
\begin{center}
\url{https://bitbucket.org/amiede/classicthesis/}
\end{center}
Happy users of \texttt{classicthesis} usually send a real postcard to the author, a collection of postcards received so far is featured here: 
\begin{center}
\url{http://postcards.miede.de/}
\end{center}
 
\bigskip

\noindent\finalVersionString

%Hermann Zapf's \emph{Palatino} and \emph{Euler} type faces (Type~1 PostScript fonts \emph{URW
%Palladio L} and \emph{FPL}) are used. The ``typewriter'' text is typeset in \emph{Bera Mono}, 
%originally developed by Bitstream, Inc. as ``Bitstream Vera''. (Type~1 PostScript fonts were made 
%available by Malte Rosenau and
%Ulrich Dirr.)

%\paragraph{note:} The custom size of the textblock was calculated
%using the directions given by Mr. Bringhurst (pages 26--29 and
%175/176). 10~pt Palatino needs  133.21~pt for the string
%``abcdefghijklmnopqrstuvwxyz''. This yields a good line length between
%24--26~pc (288--312~pt). Using a ``\emph{double square textblock}''
%with a 1:2 ratio this results in a textblock of 312:624~pt (which
%includes the headline in this design). A good alternative would be the
%``\emph{golden section textblock}'' with a ratio of 1:1.62, here
%312:505.44~pt. For comparison, \texttt{DIV9} of the \texttt{typearea}
%package results in a line length of 389~pt (32.4~pc), which is by far
%too long. However, this information will only be of interest for
%hardcore pseudo-typographers like me.%
%
%To make your own calculations, use the following commands and look up
%the corresponding lengths in the book:
%\begin{verbatim}
%    \settowidth{\abcd}{abcdefghijklmnopqrstuvwxyz}
%    \the\abcd\ % prints the value of the length
%\end{verbatim}
%Please see the file \texttt{classicthesis.sty} for some precalculated 
%values for Palatino and Minion.
%
%    \settowidth{\abcd}{abcdefghijklmnopqrstuvwxyz}
%    \the\abcd\ % prints the value of the length






==> FrontBackmatter/Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}
Put your declaration here.
\bigskip
 
\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{5cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}


==> FrontBackmatter/DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip                        

    \begingroup
        \color{Maroon}\spacedallcaps{\myTitle}
    \endgroup
\end{center}        


==> FrontBackmatter/Publications.tex <==
%*******************************************************
% Publications
%*******************************************************
\pdfbookmark[1]{Publications}{publications}
\chapter*{Publications}\graffito{This is just an early --~and currently ugly~-- test!}
This might come in handy for PhD theses: some ideas and figures have appeared previously in the following publications:

%\noindent Put your publications from the thesis here. The packages \texttt{multibib} or \texttt{bibtopic} etc. can be used to handle multiple different bibliographies in your document.

\begin{refsection}[ownpubs]
    \small
    \nocite{*} % is local to to the enclosing refsection
    \printbibliography[heading=none]
\end{refsection}

\emph{Attention}: This requires a separate run of \texttt{bibtex} for your \texttt{refsection}, \eg, \texttt{ClassicThesis1-blx} for this file. You might also use \texttt{biber} as the backend for \texttt{biblatex}. See also \url{http://tex.stackexchange.com/questions/128196/problem-with-refsection}.
